Continuous grey model with conformable fractional derivative

The existing fractional grey prediction models mainly use discrete fractional-order difference and accumulation, but in the actual modeling, continuous fractional-order calculus has been proved to have many excellent properties, such as hereditary. Now there are grey models established with continuous fractional-order calculus method, and they have achieved good results. However, the models are very complicated in the calculation and are not conducive to the actual application. In order to further simplify and improve the grey prediction models with continuous fractional-order derivative, we propose a simple and effective grey model based on conformable fractional derivatives in this paper, and two practical cases are used to demonstrate the validity of the proposed model.

==> dic.tex <==
\bibitem{1}
Abdeljawad T, Al-Mdallal QM. Discrete Mittag-Leffler kernel type fractional difference initial value problems and Gronwalls inequality. J Comput Appl Math 2018;339:218–30. 

\bibitem{2}
Abdeljawad T, Al-Mdallal QM, Jarad F. Fractional logistic models in the frame of fractional operators generated by conformable derivatives. Chaos Solit Fract 2019;119:94–101.

\bibitem{3}
Al-Mdallal QM. On fractional-Legendre spectral Galerkin method for fractional Sturm–Liouville problems. Chaos Solit Fract 2018;116:261–7. 

\bibitem{4}
Al-Mdallal QM, Hajji MA. A convergent algorithm for solving higher-order nonlinear fractional boundary value problems. Fract Calcul Appl Anal 2015;18(6):1423–40. 

\bibitem{5}
Al-Mdallal Q, Abro KA, Khan I. Analytical solutions of fractional Walters b fluid with applications. Complexity 2018;2018. 

\bibitem{6}
Al-Mdallal QM, Hajji MA. A convergent algorithm for solving higher-order nonlinear fractional boundary value problems. Fract Calcul Appl Anal 2015;18(6):1423–40.

\bibitem{7}
Al-Mdallal QM, Omer ASA. Fractional-order legendre-collocation method for solving fractional initial value problems. Appl Math Comput 2018;321:74–84. 

\bibitem{8}
Al-Mdallal QM, Syam MI. An efficient method for solving non-linear singularly perturbed two points boundary-value problems of fractional order. Commun Nonlinear Sci Numer Simul 2012;17(6):2299–308.

\bibitem{9}
Scherer, Rudolf, Kalla, Shyam L, Tang, Yifa,et al. The Grunwald-Letnikov method for fractional differential equations. computers & mathematics with applications, 2011, 62(3):902-917.

\bibitem{10}
WANG, Bing. S-asymptotically -periodic Solutions of R-L Fractional Derivative-Integral Equation[J]. Technology Vision, 2015(17):155-155.

\bibitem{11}
Wang J , Lv L , Zhou Y . Ulam stability and data dependence for fractional differential equations with Caputo derivative[J]. Electronic Journal of Qualitative Theory of Differential Equations, 2011, 63(63).

\bibitem{12}
S.F. Liu, Y.J. Yang, J. Forrest, Grey Data Analysis: Methods, Models and Applications, Springer Press, 2016

\bibitem{13}
LI Riyun, WANG Li, ZHANG Shuangcheng. Study of the application of grey forecast model in settlement forecast of high buildings[J]. journal of earth science & enivronmental, 2005, 27(1):84-87.

\bibitem{14}
Cao C, Gu X. The application of grey dynamic Verhulst metabolism model in the prediction of products' prices and demands[J]. INFORMATION AND CONTROL-SHENYANG-, 2005, 34(4): 398.

\bibitem{15}
ZHANG Qiuming, ZHU Hongli. Application of grey model and neural network in stock prediction[J]. computer engineering & applications, 2013, 49(12):242-236.

\bibitem{16}
Xin M , Zhibin L , Yong W . Application of a novel nonlinear multivariate grey Bernoulli model to predict the tourist income of China[J]. Journal of Computational & Applied Mathematics, 2018:S0377042718304709-.

\bibitem{17}
Wu W , Ma X , Zeng B , et al. Prediction short-term renewable energy consumption of China using a novel fractional nonlinear grey Bernoulli model[J]. Renewable Energy, 2019.

\bibitem{18}
Zeng B , Li C . Prediction the natural gas demand in China using a self-adapting intelligent grey model[J]. Energy, 2016, 112:810-825.

\bibitem{19}
Wu L , Zhao H . Prediction Air Quality Indicators for 33 Cities in China[J]. Clean Soil Air Water, 2019.

\bibitem{20}
Ding S, Dang Y G, Li X M, et al. Prediction Chinese CO2 emissions from fuel combustion using a novel grey multivariable model[J].Journal of Cleaner Production, 2017, 162: 1527-1538.

\bibitem{21}
Xie N M , Liu S F . Discrete grey prediction model and its optimization[J]. Applied Mathematical Modelling, 2009, 33(2):1173-1186.

\bibitem{22}
Cui J , Liu S F , Zeng B , et al. A novel grey prediction model and its optimization[J]. Applied Mathematical Modelling, 2013, 37(6):4399-4406.

\bibitem{23}
C.I. Chen, Application of the novel nonlinear grey Bernoulli model for prediction unemployment rate, Chaos Solitions Fractals 37 (2008) 278–287.

\bibitem{24}
Wu L , Liu S , Yao L , et al. Grey system model with the fractional order accumulation[J]. Communications in Nonlinear Science & Numerical Simulation, 2013, 18(7):1775-1785.

\bibitem{25}
Ma X , Wu W , Zeng B , et al. The conformable fractional grey system model[J]. 2018.

\bibitem{26}
Zeng B , Liu S , Cuevas C . A self-adaptive intelligence grey prediction model with the optimal fractional order accumulating operator and its application[J]. Mathematical Methods in the Applied Sciences, 2017.

\bibitem{27}
Wei B , Xie N , Hu A . Optimal solution for novel grey polynomial prediction model[J]. Applied Mathematical Modelling, 2018, 62(OCT.):717-727.

\bibitem{28}
Liu, X.M., Xie, N.M., 2019. A nonlinear grey prediction model with double shape parameters and its application. Appl. Math. Comput. 360, 203–212.

\bibitem{29}
Wang Z X , Hipel K W , Wang Q , et al. An optimized NGBM(1.1) model for prediction the qualified discharge rate of industrial wastewater in China[J]. Applied Mathematical Modelling, 2011, 35(12):p.5524-5532.

\bibitem{30}
Zhao D, Pan X, Luo M. A new framework for multivariate general conformable fractional calculus and potential applications[J]. Physica A: Statistical Mechanics and its Applications, 2018, 510: 271-280..

\bibitem{31}
Wang J , Wen Y , Gou Y , et al. Fractional-order gradient descent learning of BP neural networks with Caputo derivative[J]. Neural Networks, 2017, 89:19-30.

\bibitem{32}
Khalil R , Horani M A , Yousef A , et al. A new definition of fractional derivative[J]. Journal of Computational & Applied Mathematics, 2014, 264(5):65–70.

\bibitem{33}
X. Ma, W. Wu, B. Zeng, Y. Wang, X. Wu, The conformable fractional grey system model, ISA Transactions, 2019, doi.org/10.1016/j.isatra. 2019.07.009

\bibitem{34}
WU Lifeng, LIU Sifeng, YAO Ligen. Grey model with Caputo fractional order derivative[J]. Systems Engineering-Theory & Practice, 2015.

\bibitem{35}
Gene H, Charles C. Matrix computations. The Johns Hopkins University Press, Baltimore and London,1996.

\bibitem{36}
Wu WQ, Ma X, Zhang YY, et al. A novel conformable fractional non-homogeneous grey model for prediction carbon dioxide emissions of BRICS countries. Science of The Total Environment 2020; 707: 385 135447.

\bibitem{37}
Mirjalili, S., Lewis, A., 2016. The whale optimization algorithm. Adv. Eng. Softw. 95, 51–67.
